On learning history based policies for controlling Markov decision processes

Reinforcementlearning(RL)folkloresuggeststhathistory-basedfunctionapproximationmethods,suchas recurrent neural nets or history-based state abstraction, perform better than their memory-less counterparts, due to the fact that function approximation in Markov decision processes (MDP) can be viewed as inducing a Partially observable MDP. However, there has been little formal analysis of such history-based algorithms, as most existing frameworks focus exclusively on memory-less features. In this paper, we introduce a theoretical framework for studying the behaviour of RL algorithms that learn to control an MDP using history-based feature abstraction mappings. Furthermore, we use this framework to design a practical RL algorithm and we numerically evaluate its effectiveness on a set of continuous control tasks.

==> sections/algorithm-b.tex <==
We first consider optimizing the AIS-generator as follows: (i)~use parametric families of functions/distributions to model each component of the recursively updatable AIS generator (history-based feature map $\aisfunction_\timestep$, the update function $\hat f$, the reward predictor $\hat \cost$, and the transition kernel $\hat \transition$); (ii)~consider a weighted average of $(\hat \cost(Z_t, A_t) - \cost(S_t, A_t))^2$ and $d_{\mathfrak{F}}(\hat P(\cdot | Z_t, A_t), P(\cdot | S_t, A_t))^2$ as an auxiliary loss; (iii)~use gradient descent to optimize the AIS-generator. 


\begin{wrapfigure}{R}{0.6\textwidth}
  %\vskip -2\baselineskip
  \centering
  \includegraphics[width=0.55\textwidth]{Results/schematic.png}
  \caption{Algorithm/Agent architecture} \label{fig:blk-diag}
\end{wrapfigure} 
We use a time-series approximator such as LSTM or GRU to represent the history-based feature maps. The internal layer of such recurrent neural networks automatically acts as the update function $\hat f$. We use a multilayerd perception (MLP) layer to represent the reward approximator $\hat \cost$ and use an appropriate class of kernel approximators such as softmax or a mixture of Gaussians to represent $\hat \transition$. Let $\zeta$ denote the parameters of all components of the AIS-generator. The loss function for the AIS-generator may written as
\begin{equation}
  \aisloss(\aisparams) = \frac{1}{\Timestep}\sum_{t = 0}^{\Timestep}\Big(
    \lambda (\hat{\cost}(\Ais_{\timestep}, \Action_\timestep; \aisparams)  - \cost(\State_\timestep, \Action_\timestep))^{2} 
  + (1-\lambda) \ipm(\hat\transition(\cdot | \Ais_\timestep, \Action_\timestep\ ;\aisparams),\transition(\cdot | \State_\timestep, \Action_\timestep)^{2}\Big),\label{eq:ais-loss}
\end{equation}
where $\Timestep$ is the length of the episode or the rollout length and $\lambda \in (0,1)$ is a hyper-parameter. 

We can combine the learning of the parameters of the AIS-generator with a policy-gradient algorithm using multi-timescale stochastic approximation~\cite{borkar2008stochastic}. In particular, let $\mu(\cdot;\actorparams):\aisspace \to \Delta(\actionspace)$ be a parameterised stochastic policy with parameters $\actorparams$. Let $\performance(\actorparams,\aisparams)$ denote the performance of the policy $\mu(\cdot ;\ \actorparams)$. The policy gradient theorem~\citep{pgt,Williams2004SimpleSG,baxter-bartlett} states that for a rollout horizon $\Timestep$, we can estimate $\grad_\actorparams \performance$ as $\hat \grad_{\actorparams}\performance(\actorparams_\timestep,\aisparams_\timestep) = \sum_{\timestep=1}^{\Timestep}\discount^{\timestep-1}\cost_{\timestep}(\sum_{\tau =1}^{\timestep}\grad_{\actorparams}\log(\mu(\Action_\timestep|\Ais_\timestep ;\ \actorparams_\timestep)))$. Following a rollout of length $\Timestep$, we can then update the parameters $\{(\aisparams_i, \actorparams_i  )\}_{i \geq 1}$ as follows:
    \begin{subequations}\label{eq:pgt-update}
             \begin{align}
                \aisparams_{i+1} = \aisparams_i + \aislr_i \grad_\aisparams\aisloss(\aisparams_i), &&
                \actorparams_{i+1} = \actorparams_i + \actorlr_i \hat\grad_{\actorparams}\performance(\actorparams_{i},\aisparams_{i})\label{eq:actor-update},
            \end{align}
    \end{subequations}
    where the step-size $\{\aislr_{i}\}_{i \geq 0}$ and $\{\actorlr_{i}\}_{i \geq 0}$ satisfy the standard conditions: $\sum_{i} \aislr_{i} = \infty$, $\sum_{i}\aislr_{i}^{2}< \infty$, $\sum_{i} \actorlr_{i} = \infty$ and $\sum_{i}\actorlr_{i}^{2}< \infty$. Moreover, one can ensure that the AIS generator converges faster by choosing an appropriate $\actorlr$ such that, $\lim_{i \to \infty} \frac{\actorlr_{i}}{\aislr_{i}} = 0$. Moreover, we can use similar ideas to develop an Actor-Critic algorithm. As such, in addition to a parameterised policy $\policy(\cdot; \actorparams)$ and AIS generator $(\aisfunction_\timestep(\cdot;\aisparams), \hat f, \hat r, \hat\transition)$ we can also a parameterised critic $\hat\valuefunction(\cdot;\criticparams):\featurespace \to \real$, where $\criticparams$ are the parameters for the critic. 

==> sections/algorithm.tex <==
\section{Algorithm}\label{sec:algorithm}
    \begin{figure}[thb]
      \centerline{\includegraphics[width=\columnwidth]{Results/schematic.png}}
      \caption{Algorithm/Agent architecture} \label{fig:blk-diag}
    \end{figure}
    lalal
    The previous section helps us establish two results, the first result tells that a history-based representation can be called an AIS if it is able to evolve like a state and approximately predict the instantaneous reward and state transition. The second result tells us that if a policy is obtained using an AIS, then its performance loss is bounded in terms of the approximation error as in \eqref{eq:ais-bound}. 
    In this section we will show how one can design a theoretically grounded computational framework that uses an RL algorithm to simultaneously learn an AIS and a policy. The key idea is to represent the AIS generator and the policy using a parametric family of functions/distributions and training them using a multi-timescale optimisation algorithm. 
    
    According to \Cref{def:ais}, the AIS generator consists of four components, a compression function $\aisfunction_\timestep$, the update function $\hat f$, an approximate reward predictor $\hat \cost$, and transition kernel $\hat \transition$. We can represent the history compression function using any time series approximators such as LSTMs or GRUs. An advantage of such memory based neural networks is that their internal layers are updated in a state-like manner. Therefore, we can satisfy \Cref{def:state-update} since $\Ais_\timestep$ evolves according to the RNN's state update function such that $\hat{f} \colon \aisspace \times \statespace \times \actionspace \to \aisspace$.
     
    The main function of $\hat \cost$ and $\hat \transition$ is ensure that $\Feature_\timestep$ satisfies properties P1 and P2 (in \Cref{def:ais}), ~\ie, prediction of the instantaneous reward with a bounded error $\epsilon$ and approximation of the ground MDP's transition function with a bounded error $\delta$. One way in which the computational framework can satisfy these is conditions is by explicitly optimising the AIS generator for the constants $\epsilon$ and $\delta$. We can achieve this by modelling the reward predictor $\hat \cost$ using a multilayered perception (MLP) layer which uses the representation $\Feature_\timestep$ and action $\Action_\timestep$ to predict the approximate reward. In the same way, we can model the approximate transition kernel $\hat \transition$ using an appropriate class of stochastic kernel approximators \eg, a softmax function or a mixture of Gaussian's to learn a parametric approximation of $\transition$. We can then train the AIS generator by minimising an appropriate objective function.
     
     To make things more concrete, let us denote the AIS generator as the following collection: $\{\aisfunction_\timestep(\cdot;\aisparams), \hat{f}(\cdot;\aisparams), f_{\hat{\cost}}(\cdot;\aisparams), f_{\hat{\transition}}(\cdot:\aisparams)\}$ where $f_{\hat \cost}(\cdot;\aisparams):
     \aisspace \times \actionspace \to \real$ and $f_{\hat \transition}(\cdot;\aisparams):\aisspace \times \actionspace \to \Delta(\statespace)$ are the reward and transition approximators, and $\aisparams$ are the parameters of the respective sub-components. Instead of separately optimising the reward prediction loss $\vert \cost(\State_\timestep, \Action_\timestep) - \hat\cost (\Ais_\timestep, \Action_\timestep)\vert$, and the transition loss $\ipm(\transition, \hat \transition)$ we can combine them in a single objective function objective function as: 
     
      \begin{align}
                \aisloss(\aisparams) &= \frac{1}{\Timestep}\sum_{t = 0}^{\Timestep}\bigg( \lambda \underbrace{(f_{\hat{\cost}}(\Ais_{\timestep}, \Action_\timestep; \aisparams)  - \cost(\State_\timestep, \Action_\timestep))^{2}}_{\loss_{\hat{\Cost}} \approx \epsilon} 
                + (1-\lambda)\cdot \underbrace{\ipm(f_{\hat\transition}(\Ais_\timestep, \Action_\timestep\ ;\aisparams),\transition)^{2}}_{\loss_{\hat\transition} \approx \delta}\bigg),\label{eq:ais-loss}
    \end{align}
    where, $\Timestep$ is the length of the episode or the rollout length, $\lambda \in [0,1]$ is a hyper-parameter, reward prediction loss $\loss_{\hat{\Cost}}(;\aisparams)$ is simply the mean-squared error between the predicted and the observed reward, whereas the transition prediction loss $\loss_{\hat{\transition}}(\cdot; \aisparams)$ is the distance between predicted and observed transition distributions $\hat\transition$ and $\transition$. To compute $\loss_{\hat{\transition}}(\cdot; \aisparams)$, we need to choose an IPM. In principle we can pick any IPM, but we would want to use an IPM using which the distance $d_{\mathfrak{F}}$ can be efficiently computed.
     
    %  Besides the AIS generator the system also consists of a parametric representation of the decision policy $\mu{}(\cdot \ ; \actorparams)$, where $\actorparams$ represent the policy parameters. The schematic of our system architecture is given in \Cref{fig:blk-diag}. 
    
    \subsection{Choice of an IPM} \label{sec:ipm-choice}
    
        To compute the IPM $d_\mathfrak{F}$ we need to know the probability density functions $\hat \transition$ and $\transition$. As we assume $\hat \transition$ to belongs to a parametric family, we know its density function closed form. However, since we are in the learning setup, we can only access samples from $\transition $. 
    
        For a function a $f\in \mathfrak{F}$, and probability density functions $\transition$ and $\hat \transition$ such that, $\nu_1 = \transition$, and $\nu_2 =\hat \transition$, we can estimate the IPM $d_\mathfrak{F}$ between a distribution and samples using the duality $|\int_\aisspace f d\nu_1 - \int_\aisspace f d\nu_2|$.
        
        In this paper, we use two from of IPMs, the MMD distance and the Wasserstein/Kantorovich–Rubinstein distance. 
        \vspace{-10pt}
        \paragraph{MMD Distance:} Of the two alternatives, MMD distance is the easier compute as we can use some of its properties to simply its computation. Towards that end, when $\hat \transition$ is a real-valued distribution that can be characterised by its mean $m_\aisparams$, the MMD-based AIS loss can be given as:
        \begin{align}
            \aisloss(\aisparams) &= \frac{1}{\Timestep}\sum_{t = 0}^{\Timestep}\bigg( \lambda (f_{\hat{\cost}}(\Ais_{\timestep}, \Action_\timestep; \aisparams)  - \cost(\State_\timestep, \Action_\timestep))^{2} 
            + (1-\lambda)(m^{\State_\timestep}_{\aisparams} - 2\State_\timestep)^{\top}m^{\State_\timestep}_{\aisparams}  \bigg),\label{eq:mmd-ais-loss}
        \end{align}
        where $m^{\State_\timestep}_{\aisparams}$ is obtained using the from the transition approximator, ~\ie, the mapping $f_{\hat\transition}(\aisparams): \aisspace \times \actionspace \to \real$. For the detailed derivation of the above loss see \Cref{sec:mmd-details}
        \vspace{-5pt}
        \paragraph{Wasserstein/Kantorovich–Rubinstein distance:}
        When $\ipm$ is the Wasserstein/Kantorovich–Rubinstein distance, we can compute it by solving a linear program~\citep{Sriperumbudur}. In some settings, it might be computationally expensive to solve a linear program at each time step before updating the parameters $\aisparams$. Therefore, we propose to approximate the Wasserstein distance using a KL-divergence~\citep{kl} based upper-bound. The KL divergence based AIS loss is given as:
          \begin{align}
                \aisloss(\aisparams) &= \frac{1}{\Timestep}\sum_{t = 0}^{\Timestep}\bigg( \lambda (f_{\hat{\cost}}(\Ais_{\timestep}, \Action_\timestep; \aisparams)  - \cost(\State_\timestep, \Action_\timestep))^{2}
                + (1-\lambda)\log(\hat \transition(\State_\timestep;\aisparams))  \bigg),\label{eq:w-ais-loss}
            \end{align}
        where, $d_{\mathfrak{F}^{\text{W}}}^{2}(\transition, \hat \transition)\leq \log(\hat \transition(\State_\timestep;\aisparams))$ is the KL-divergence based upper bound. For the details of this derivation see \Cref{sec:wass-details}. 
  
  
        
        % When $\ipm$ is the Wasserstein/Kantorovich–Rubinstein distance, we can compute it by solving a linear program~\citep{Sriperumbudur}. In some settings, it might be computationally expensive to solve a linear program at each time step before updating the parameters $\aisparams$. 
        % Therefore, we propose to use the a Sinkhorn divergence~\citep{Sinkhorn1967DiagonalET} based estimator to compute the Wasserstein distance. For a detailed discussion on this topic we refer the reader to the large body of work in the field of optimal transport~\citep{Cuturi13, Knight08, RamdasTC17, GenevayPC18}. As these technicalities are not relevant to the scope of this paper, we will define the Sinkhorn divergence based estimator as follows:
        % \begin{align}
        %     \nu_1 = \sum_{i=1}^{N} \nu_{1_{i}}\delta_{X_{i}} && \nu_2 = \sum_{i=1}^{N} \nu_{2_{i}}\delta_{W_{i}},
        % \end{align}
        % where $\nu_1, \nu_2 \in \real^{N}$ and $X, W \in \real^{N \times D}$
        % \begin{align}\label{eq:OT}
        %     S_{\epsilon}(\nu_1, X, \nu_2, W) &= \sum_{i=1}^{N} \nu_{1_{i}}(j_{i} - k_{i}) + \sum_{i=1}^{N} \nu_{2_{i}}(y_{i} - g_{i})
        % \end{align}
        % where
        % \begin{align}
        %     j_i &= - \epsilon \log \bigg(\sum_{i'=1}^{N} \exp(\log(\nu_{2_{i'}} + \frac{1}{\epsilon}y_{i'} - \frac{1}{\epsilon}C(X_i, W_{i'}))\bigg)\\
        %     y_i &= - \epsilon \log \bigg(\sum_{i'=1}^{N} \exp(\log(\nu_{1_{i'}} + \frac{1}{\epsilon}j_{i'} - \frac{1}{\epsilon}C(X_{i'}, W_i))\bigg)\\
        %     k_i &= - \epsilon \log \bigg(\sum_{i'=1}^{N} \exp(\log(\nu_{1_{i'}} + \frac{1}{\epsilon}k_{i'} - \frac{1}{\epsilon}C(X_i, X_{i'}) )\bigg)\\
        %     g_i &= - \epsilon \log \bigg(\sum_{i'=1}^{N} \exp(\log(\nu_{2_{i'}} + \frac{1}{\epsilon}g_{i'} - \frac{1}{\epsilon}C(W_i, W_{i'}) )\bigg)
        % \end{align}
    
   \subsection{Policy gradient algorithm}\label{sec:pgt}
        Following the design of the auxiliary algorithmic modules, we now provide a policy-gradient algorithm to learning both the AIS and policy. The schematic of our agent architecture is given in \Cref{fig:blk-diag}, and pseudo-code is given in \Cref{alg:ciac-a}.
        
        Given an AIS $\Ais$, we can simultaneously learn the AIS-generator and the policy using a multi-timescale stochastic gradient ascent algorithm~\citep{borkar2008stochastic}. Let $\mu(\cdot;\actorparams):\aisspace \to \Delta(\actionspace)$ be a parameterised stochastic policy with parameters $\actorparams$. Let $\performance(\actorparams,\aisparams)$ denote the performance of the policy $\mu(\cdot ;\ \actorparams)$. The policy gradient theorem~\citep{pgt,Williams2004SimpleSG,baxter-bartlett} states that: 
        % \begin{align*}
        %     \grad_{\actorparams}\performance(\actorparams_\timestep,\aisparams_\timestep) &= \expecun{}\bigg[\sum_{\timestep=1}^{\infty}\discount^{\timestep-1}\cost_{\timestep}\bigg(\sum_{\tau =1}^{\timestep}\grad_{\actorparams}\log(\mu(\Action_\timestep|\Ais_\timestep ;\ \actorparams_\timestep))\bigg)\bigg].\label{eq:pg}
        % \end{align*}
        For a rollout horizon $\Timestep$, we can estimate $\grad_\actorparams \performance$ as:
        \begin{align*}
            \hat \grad_{\actorparams}\performance(\actorparams_\timestep,\aisparams_\timestep) &= \sum_{\timestep=1}^{\Timestep}\discount^{\timestep-1}\cost_{\timestep}\bigg(\sum_{\tau =1}^{\timestep}\grad_{\actorparams}\log(\mu(\Action_\timestep|\Ais_\timestep ;\ \actorparams_\timestep))\bigg).
        \end{align*}
        Following a rollout of length $\Timestep$, we can then update the parameters $\{(\aisparams_i, \actorparams_i  )\}_{i \geq 1}$ as follows:
        \begin{subequations}\label{eq:pgt-update}
             \begin{align}
                \aisparams_{i+1} &= \aisparams_i + \aislr_i \grad_\aisparams\aisloss(\aisparams_i)\label{eq:ais-update},\\
                \actorparams_{i+1} &= \actorparams_i + \actorlr_i \hat\grad_{\actorparams}\performance(\actorparams_{i},\aisparams_{i})\label{eq:actor-update},
            \end{align}
        \end{subequations}
       
         where the step-size $\{\aislr_{i}\}_{i \geq 0}$ and $\{\actorlr_{i}\}_{i \geq 0}$ satisfy the standard conditions $\sum_{i} \aislr_{i} = \infty$, $\sum_{i}\aislr_{i}^{2}< \infty$, $\sum_{i} \actorlr_{i} = \infty$ and $\sum_{i}\actorlr_{i}^{2}< \infty$ respectively. Moreover, one can ensure that the AIS generator converges faster by choosing an appropriate $\actorlr$ such that, $\lim_{i \to \infty} \frac{\actorlr_{i}}{\aislr_{i}} = 0$.
         
         Note that we can use similar ideas to develop an Actor-Critic algorithm. As such, in addition to a parameterised policy $\policy(\cdot; \actorparams)$ and AIS generator $(\aisfunction_\timestep(\cdot;\aisparams), \hat f, \hat r, \hat\transition)$ we can also a parameterised critic $\hat\valuefunction(\cdot;\criticparams):\featurespace \to \real$, where $\criticparams$ are the parameters for the critic. The details of the Actor Critic Algorithm can be found in \Cref{sec:AC}, and the convergence analysis of both algorithms can be found in \Cref{sec:convergence}.
        
     
        \begin{algorithm}[t]
            \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
            \SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
            \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
            \SetAlgoLined
            \Input{$\iota_{0}$: Initial state distribution,\\
                  $\aisparams_{0}$: Ais parameters,\\
                  $\actorparams_{0}$: Actor parameters,\\ 
                %   $\criticparams_{0}$: Critic parameters,
                %   $\ais_{0}$: Initial Ais, 
                  $\action_{0}$: Initial action,\\
                  $\mathcal{D} = \emptyset$: Replay buffer,\\
                  $N_{\text{comp}}$: Computation budget,\\
                  $N_{\text{ep}}$: Episode length,\\
                  $N_{\text{grad}}$: Gradient steps}
            % \KwResult{Write here the result }
             \For{iterations $i = 0:N_{\text{comp}}$ }{
                  Sample start state $\sts_{0}\sim \iota_{0}$\;
                  \For{iterations $j = 0:N_{\text{ep}}$ }
                  {
                    
                  $\ais_{j} = \aisfunction_{\aisparams}(\sts_{1:j},\action_{1:j-1})$\ \tcp*{\tiny{final layer of a GRU cell.}}
                  $\action_{j} = \mu_{\actorparams}(\ais_{j})$\;
                  $\sts_{j+1} = \transition(\sts_{j},\action_{j})$\ \tcp{\tiny{sample next state from the MDP.}}
                  $\mathcal{D} \subseteq \{\ais_{j},\action_{j},\sts_{j},\sts_{j+1}\}$\;
                  $\action_{j-1} = \action_{j}$\;
                  $\sts_{j} = \sts_{j+1}$\;
                  }
                  \For{every batch $b \in \mathcal{D}$}
                  {
                        \For {gradient step $t=0:N_{\text{grad}}$}
                        {
                        %  $\aisparams_{\timestep+1,b,\valuefunction} = \aisparams_{\timestep,b,\valuefunction} + \aislr  \grad_{\aisparams_{\valuefunction}}\aisloss(\aisparams_{\timestep,b,\valuefunction})$\;
                        %  $\criticparams_{\timestep+1,b} = \criticparams_{\timestep,b} + \criticlr\grad_{\criticparams}\criticloss(\criticparams_{\timestep,b})$\;
                         $\aisparams_{\timestep+1,b} = \aisparams_{\timestep,b} + \aislr \grad_{\aisparams}\aisloss(\aisparams_{\timestep,b})$\;
                         $\actorparams_{\timestep+1,b} = \actorparams_{\timestep,b} +\actorlr \hat\grad_{\actorparams}\performance(\actorparams_{\timestep,b},\aisparams_{\timestep,b})$
                        }
                  }
             }
          \caption{Policy Search with AIS }\label{alg:ciac-a}
      \end{algorithm}

==> sections/model-new.tex <==
\section{Background and Motivation}\label{sec:background}
        \begin{figure*}[!ht]
          \centering
          \begin{minipage}{0.75\linewidth}
          \subfigure[$P(0)$]{
            \begin{tikzpicture}[thick,scale=0.65]
              \node [agent] at (0, 0) (0) {$0$};
              \node [agent] at (1, 0) (1) {$1$}; 
              \node [agent] at (0, 1) (3) {$3$};
              \node [agent] at (1, 1) (2) {$2$};
              \path[->]
                    (0) edge node[below] {$0.5$} (1)
                    (1) edge node[right] {$0.5$} (2)
                    (2) edge node[above] {$0.5$} (3)
                    (3) edge node[left]  {$0.5$} (0)
                    (0) edge[loop left] node {$0.5$} (0)
                    (1) edge[loop right] node {$0.5$} (1)
                    (2) edge[loop right] node {$0.5$} (2)
                    (3) edge[loop left] node {$0.5$} (3)
                    ;
            \end{tikzpicture}}
           \hfill
          \subfigure[$P(1)$]{
            \centering
            \begin{tikzpicture}[thick,scale=0.75]
              \node [agent] at (0, 0) (0) {$0$};
              \node [agent] at (1, 0) (1) {$1$}; 
              \node [agent] at (0, 1) (3) {$3$};
              \node [agent] at (1, 1) (2) {$2$};
              \path[<-]
                    (0) edge node[below] {$0.5$} (1)
                    (1) edge node[right] {$0.5$} (2)
                    (2) edge node[above] {$0.5$} (3)
                    (3) edge node[left]  {$0.5$} (0)
                    (0) edge[loop left] node {$0.5$} (0)
                    (1) edge[loop right] node {$0.5$} (1)
                    (2) edge[loop right] node {$0.5$} (2)
                    (3) edge[loop left] node {$0.5$} (3)
                    ;
            \end{tikzpicture}}
            \hfill
            \subfigure[$P(2)$]{%
                  \begin{tikzpicture}[thick,scale=0.65]
                  \node [agent] at (0, 0) (0) {$0$};
                  \node [agent] at (1, 0) (1) {$1$}; 
                  \node [agent] at (0, 1) (3) {$3$};
                  \node [agent] at (1, 1) (2) {$2$};
                  \path[->]
                        (0) edge [bend right] node[below] {$0.5$} (1)
                        (1) edge [bend right] node[right] {$0.5$} (2)
                        (2) edge [bend right] node[above] {$0.5$} (3)
                        (3) edge [bend right] node[left]  {$0.5$} (0)
                        (0) edge [bend right] node[right] {} (3)
                        (3) edge [bend right] node[below] {} (2)
                        (2) edge [bend right] node[left]  {} (1)
                        (1) edge [bend right] node[above]  {} (0);
                \end{tikzpicture}}
                \caption{The transition probability model for the example of}
          \label{fig:P}
          \end{minipage}%
          \begin{minipage}{0.25\linewidth}
          \centering
            \begin{tikzpicture}[thick,scale=0.9]
              \node [agent] at (0, 0) (0) {$0$};
              \node [agent] at (1, 0) (1) {$1$}; 
              \node [agent] at (0, 1) (3) {$3$};
              \node [agent] at (1, 1) (2) {$2$};
              \path[->]
                    (0) edge node[below] {$0.5$} (1)
                    (1) edge[bend right] node[right] {$0.5$} (2)
                    (2) edge[bend right]  node[left] {$0.5$} (1)
                    (3) edge node[left]  {$0.5$} (0)
                    (3) edge node[above] {$0.5$} (2)
                    (0) edge[loop left] node {$0.5$} (0)
                    (1) edge[loop right] node {$0.5$} (1)
                    (2) edge[loop right] node {$0.5$} (2)
                    (3) edge[loop left] node {$0.5$} (3)
                    ;
            \end{tikzpicture}
          \caption{The transition probability of the optimal policy}
          \label{fig:optimal}
          \end{minipage}
        \end{figure*}

    % \subsection{Function approximation in MDPs}
    
        Consider an MDP $ \mdp = \langle \statespace, \actionspace, \transition, \cost, \discount \rangle$ where $\statespace$ denotes the state space, $\actionspace$ denotes the action space, $\transition$ denotes the controlled transition matrix, $\cost \colon \statespace \times \actionspace \to \real$ denotes the per-step reward, and $\discount \in (0,1)$ denotes the discount factor.
                
        The performance of a randomised (and possibly history-dependent) policy $\policy$
        starting from a start state $\sts_{0}$ is measured by the value function, defined as:
        \begin{equation}
          \valuefunction^{\policy}(\sts_0) = \expecun{}^{\policy}\bigg[\sum_{\timestep=0}^{\infty}\discount^{\timestep}\cost(\State_{\timestep},\Action_{\timestep}) \bigg| \State_{0} = \sts_{0}\bigg].
        \end{equation}
        A policy maximising $\valuefunction^{\policy}(\sts_0)$ over all (randomized and possibly history dependent) policies is called the optimal policy with respect to initial state $s_0$ and is denoted by $\policy^{\star}$\footnote{This notion can easily be extended to start state distributions.}.
                
        In many applications, $\statespace$ and $\actionspace$ are combinatorially large or uncountable, which makes it intractable to compute the optimal policy. 
        Most practical RL algorithms overcome this hurdle by using function approximation where the state is mapped to a feature space $\featurespace$ using a state abstraction function $\basis:\statespace \to \featurespace$. In Deep-RL algorithms, the last layer of the network is often viewed as a feature vector. These feature vectors are then used as an approximate state for approximating the value function $\hat\valuefunction: \featurespace \to \real$ and/or computing an approximately optimal policy $\mu:\featurespace \to \Delta(\actionspace)$~\citep{Sutton+Barto:1998} (where $\Delta(\actionspace)$ denotes the set of probability distribution over actions). We use $\tilde{\mu} = \mu \circ \basis$ ~\ie, $\tilde{\mu} = \mu(\phi(\cdot))$ to denote the ``flattened" policy that maps states to action distributions.
        
        % The features $\Feature_\timestep$ are then used as an approximate state for computing the value function $\hat\valuefunction: \featurespace \to \real$ and/or the policy $\mu:\featurespace \to \Delta(\actionspace)$~\citep{Sutton+Barto:1998} (where $\Delta(\actionspace)$ denotes the set of probability distribution over actions). We denote by $\mu \circ \phi $ as the ``flattened" policy that maps states to action distributions, by composing the feature abstraction and the policy acting on it. In Deep-RL algorithms, the output of the last layer of the network is often viewed as the feature vector $\Feature_{\timestep}$.
        
        % A well known yet often overlooked fact about function approximation is that the features used as a proxy state may not satisfy the controlled Markov property \ie, in general,
        A well known fact about function approximation is that the features that are used as an approximate state may not satisfy the controlled Markov property \ie, in general, 
        \[
            \prob(\Feature_{\timestep+1} \mid \Feature_{1:\timestep}, \Action_{1:\timestep}) \neq
            \prob(\Feature_{\timestep+1} \mid \Feature_\timestep, \Action_\timestep).
        \]

        To see the implications of this fact, consider the toy MDP depicted in Fig.~\ref{fig:P}, with $ \statespace = \{0, 1, 2, 3\}$, $\actionspace =
        \{0, 1, 2\}$, $\{\transition_{\sts, \sts'}(\action)\}_{\action \in \actionspace}$, and $r(0) = r(1) = -1$, $r(2) = 1$, $r(3) = -K$, where $K$ is a large positive number.
       Given the reward structure the objective of the policy is to try to avoid state~$3$ and keep the agent at state~$2$ as much as possible. It is easy to see that the optimal policy is 
            \[
              \pi^\star(0) = 0, \quad
              \pi^\star(1) = 0, \quad
              \pi^\star(2) = 1,
              \text{ and}\quad
              \pi^\star(3) = 2.
            \]
        The Markov chain induced by the optimal policy is shown in Fig.~\ref{fig:optimal}. 
        Note that if the initial state is not state~$3$ then an agent will never visit that state under the optimal policy. Furthermore, any policy which cannot prevent the agent from visiting state~$3$ will have a large negative value and, therefore, cannot be optimal.
        Now suppose the feature space $\featurespace = \{0, 1\}$. It is easy to see that for any Markovian feature-abstraction $\policyencoder{} \colon \statespace \to \featurespace$, no policy $\hat \pi \colon \featurespace \to \actionspace$ can prevent the agent from visiting state~$3$. Thus, the best policy when using Markovian feature abstraction will perform significantly worse than the optimal policy (which has direct access to the state).
    
        However, it is possible to construct a history-based feature-abstraction  $\policyencoder$ and a history-based control policy $\hat \pi$ that works with $\phi$ and is of the same quality as $\pi^\star$. For this, consider the following \emph{codebooks} (where the entries denoted by a dot do not matter):
        \begin{align*}
          F(1) &= \begin{bmatrix}
            0 & 1 & \cdot & \cdot \\
            \cdot & 0 & 1 & \cdot \\
            \cdot & \cdot & 0 & 1 \\
            1 & \cdot & \cdot & 0
          \end{bmatrix}, 
          &
          F(2) &= \begin{bmatrix}
            1 & \cdot & \cdot & 0 \\
            0 & 1 & \cdot & \cdot \\
            \cdot & 0 & 1 & \cdot \\
            \cdot & \cdot & 0 & 1
          \end{bmatrix} ,
           \\
          F(3) &= \begin{bmatrix}
            \cdot & 0 & \cdot & 1 \\
            0 & \cdot & 1 & \cdot \\
            \cdot & 0 & \cdot & 1 \\
            0 & \cdot & 1 & \cdot
          \end{bmatrix},
          &
          D(0) &= \begin{bmatrix}
            0 & 1 \\
            1 & 2 \\
            2 & 3 \\
            3 & 0 
          \end{bmatrix} ,
          \\
          D(1) &= \begin{bmatrix}
            3 & 0 \\
            0 & 1 \\
            1 & 2 \\
            2 & 3 
          \end{bmatrix} ,
          &
          D(2) &= \begin{bmatrix}
            1 & 3 \\
            0 & 2 \\
            1 & 3 \\
            0 & 2 
          \end{bmatrix} .
        \end{align*}
        Now consider the following feature-abstraction:
        \[
          Z_t =  F_{S_{t-1}, S_t}(A_{t-1}).
        \]
        and a control policy $\mu$ which is a finite state machine with memory $M_t$ that is updated as:
        \[
          M_t = D_{M_{t-1}, Z_t}(A_{t-1}).
        \]
        and chooses the actions according to:
        \[
          \quad
          A_t = \pi(M_t).
        \]
        where $\pi \colon \statespace \to \Delta(\actionspace)$ is any pre-specified reference policy. It can be verified that if the system starts from a known initial state then $\mu \circ \basis = \pi$. 
         Thus, if we choose the reference policy $\pi=\pi^\star$, then
        the agent will never visit state~$3$ under $\mu \circ \basis$, in contrast to Markovian feature-abstraction policies where (as we argued before) state~$3$ is always visited.
        
        From the above example, we can see that when system dynamics are known, one can exploit the problem structure to design history-based feature abstractions which outperform their memoryless counterparts. However, such constructions are not feasible in the general learning setup, where the system dynamics are unknown. 
        % One way to overcome this issue is to let the policy $\policy{}$ be a function of all the information available to the system at time $\timestep$  ~\ie, $\policy{}_\timestep: \historyspace_{\timestep} \to \Delta(\actionspace)$ where, $\historyspace_\timestep \define \{\statespace^{1:\timestep},\featurespace^{1:\timestep-1}, \actionspace^{1:\timestep-1}\}$. 
        We can overcome this issue by letting the policy be a function of the history of state, actions and observations observed until time $\timestep$, \ie, $\policy{}_\timestep: \historyspace_{\timestep} \to \Delta(\actionspace)$ where, $\historyspace_\timestep \define \{\statespace \times \featurespace \times \actionspace\}$. 
        
        % Since the environment is an MDP, the state $\State_\timestep$ is  a sufficient statistic and the loss of information happens when $\State_\timestep$ is mapped to $\Feature_\timestep$. This is a subtle yet critical distinction between POMDPs and function approximation in MDPs. In POMDPs the state signal is unavailable, and the system only sees a observation vector $\Feature_\timestep$. Whereas, in function approximation setup, we can observe the state signal perfectly and partial observability is induced due to feature abstraction. Therefore, we can discard the the history of states and focus on the policies of the following form $\policy{}_\timestep: \historyspace_{\timestep} \to \Delta(\actionspace)$ where, $\historyspace_\timestep \define \{\statespace,\featurespace^{1:\timestep-1}, \actionspace^{1:\timestep-1}\}$.   
        
        As the size of history grows with time $t$ and it is computationally and conceptually difficult to use it for deriving a dynamic programming decomposition. One solution is to map the history to a fixed dimensional representation and use it as a state for designing a dynamic program. One can think of such a representation as an information state~\citep{kwakernaakh.1965,infostate-Witsenhausen,Striebel1965SufficientSI,Bohlin1970InformationPF,Davis1972InformationSF,Kumar1986StochasticSE}.  Due to lossy compression a prefect information state may be hard to obtain, but we an construct an approximate information state (AIS) such that it satisfies the controlled Markov property and captures the sufficient information for identifying the policy. In the next section we will show how to construct and AIS and use it for obtaining a dynamic program, which can then be solved, either exactly or approximately, to obtain a policy with a bounded approximation error. 
        



\section{Model}\label{sec:main}

        The approximation results of our framework depend on the properties of metrics on probability spaces. In particular, we derive results for Total Variation (TV) distance, Wasserstein/Kantorovich-Rubinstein distance and Maximum-Mean Discrepancy (MMD) distance. All of these metrics are instances of Integral Probability Measures (IPMs) -- a class of metrics that have a dual characterisation. Viewing all the above metrics through the lens of IPMs allows us to derive a general approximation bound that holds for all the instances of IPMs, and then specialise the bound to specific instances \ie, TV, Wasserstein and MMD distance. Before defining our main model we will briefly describe the important properties of IPMs necessary for deriving our results.
        
        % \subsection{Integral probability metrics (IPM)}
            \begin{definition}[~\citep{ipm}]\label{def:ipm}
                    Let $(\mathcal{E},\mathcal{G})$ be a measurable space and $\mathfrak{F}$ denote a class of uniformly bounded measurable functions on $(\mathcal{E},\mathcal{G})$. The integral probability metric between two probability distributions  $\nu_1, \nu_2 \in \mathcal{P}(\mathcal{E})$ with respect to the function class $\mathfrak{F}$ is defined as:
                    \begin{align}
                        \ipm(\nu_1, \nu_2) &= \sup_{f \in \mathfrak{F}}\bigg| \int_{\mathcal{E}}f d\nu_1  - \int_{\mathcal{E}}f d\nu_2\bigg|.\label{eq:def-ipm}
                    \end{align}
                    
                    For any function $f$ (not necessarily in $\mathfrak{F}$), the Minkowski functional $\rho_{\mathfrak{F}}$ associated with the $\ipm$ is given as:
                    \begin{align}
                        \rho_{\mathfrak{F}}(f)&\define \inf\{\rho \in \real_{\geq 0}: \rho^{-1}f \in \mathfrak{F}\}.\label{eq:minkowski-functional}
                    \end{align}
                    
                    \Cref{eq:minkowski-functional}, implies that that for any function $f$:
                    \begin{align}
                         \bigg|\int_{\mathcal{E}}fd\nu_1 - \int_{\mathcal{E}}fd\nu_2 \bigg|\leq \rho_{\mathfrak{F}}(f)\ipm(\nu_1,\nu_2). \label{eq:ipm-implication}
                     \end{align}\label{eq:ipm-function-diff}
                    
            \end{definition}
            \noindent We will now list the types of IPMs used in this paper with their Minkowski functionals.
            \begin{compactitem}
                \item[1.]\label{def:tv-dist}{\bf Total Variation Distance}: If $\mathfrak{F}$ is chosen as $\mathfrak{F}^{\text{TV}} \define \{\frac{1}{2}\spn(f) = \frac{1}{2}(\max(f)- \min(f))\}$, then $\ipm$ is the total variation distance, and its Minkowski functional is: $\rho_{\mathfrak{F}^{\text{TV}}}(f) = \frac{1}{2}\spn(f)$. 
                \item[2.]\label{def:kr-dist}{\bf Wasserstein/Kantorovich-Rubinstein Distance}: If $\mathcal{E}$ is a metric space and $\mathfrak{F}$ is chosen as $\mathfrak{F}^{W} \define \{f: L_f \leq 1 \}$(where $L_f$ denotes the Lipschitz constant of $f$ with respect to the metric on $\mathcal{E}$), then $\ipm$ is the Wasserstein or the Kantorovich distance. The Minkowski function for the Wasserstein distance is a $\rho_{\mathfrak{F}^W}(f) = L_f$.
                \item[3.] \label{def:mmd-dist}{\bf Maximum Mean Discrepancy (MMD) Distance}: Let $\mathcal{U}$ be a reproducing kernel Hilbert space (RKHS) of real-valued functions on $\mathcal{E}$ and $\mathfrak{F}$ is choosen as $\mathfrak{F}^{MMD} \define \{f\in \mathcal{U}: \Vert f \Vert _{\mathcal{U}} \leq 1 \}$, (where $\Vert \cdot \Vert_{\mathcal{U}}$ denotes the RKHS norm), then $\ipm$ is the Maximum Mean Discrepancy (MMD) distance and its Minkowski functional is $\rho_{\mathfrak{F}^{\text{MMD}}}(f) = \Vert f\Vert _{\mathcal{U}}$.
            \end{compactitem}

Consider a Markov decision process (MDP) $\mdp = \langle \statespace, \actionspace, \cost, \transition, \discount \rangle$ with state-space $\statespace$, action space $\actionspace$, reward function $\cost$, transition kernel $\transition$, and discount factor $\discount$.

Let $\{\aisfunction\}_{\timestep \geq 0}$ be a family of history-dependent feature abstraction functions. We say that the features $\Ais_\timestep = \aisfunction_\timestep (\State_{1:\timestep}, \Action_{1:\timestep-1})$ are an $(\epsilon, \delta)$ \emph{approximate information state} (AIS) if there exist a  reward approximation function $\hat \cost: \aisspace \times \actionspace \to \real$ and approximate transition kernel $\hat \transition: \aisspace \times \actionspace \to \Delta(\statespace)$ which satisfy the following properties: 
(P1)~\ul{Sufficient for approximate performance evaluation:} for all $\timestep$, $ \vert \cost(\State_{\timestep}, \Action_{\timestep})- \hat{\cost}(\Feature_\timestep, \Action_\timestep)\vert \leq \epsilon \label{def:p1}$, and 
(P2) \ul{Sufficient for predicting future states approximately:} for all $\timestep$, $ d_{\mathfrak{F}}(\transition(\cdot \vert \State_\timestep, \Action_\timestep), \hat \transition(\cdot\vert \Feature_\timestep, \Action_\timestep)) \leq \delta$, where $d_{\mathfrak{F}}$ is an integral probability measure (IPM)%\footnote{Given a class $\mathfrak{F}$ of uniformly measurable functions on a measurable space $(\mathcal{E}, \mathcal{G})$, the integral probability metric (IPM) between two probability distributions  $\nu_1, \nu_2 \in \mathcal{P}(\mathcal{E})$ with respect to the function class $\mathfrak{F}$ is given by: $\ipm(\nu_1, \nu_2) = \sup_{f \in \mathfrak{F}}\vert \int_{\mathcal{E}}f d\nu_1  - \int_{\mathcal{E}}f d\nu_2\vert$~\cite{ipm}.} 
 on $\Delta(\statespace)$. We call $(\hat{\cost}, \hat \transition)$ as an $(\epsilon, \delta)$-\emph{AIS generator}.
    
%The metric $d_{\mathfrak{F}}$ captures the distance between the MDP's transition probability distribution $\transition$, and the approximate transition distribution $\hat \transition$ based on $\Ais_\timestep$,  and $\Action_\timestep$. 
% Moreover, for any function $f$ (not necessarily in $\mathfrak{F}$), the Minkowski functional $\rho_{\mathfrak{F}}$ associated with the $\ipm$ is given as: $\rho_{\mathfrak{F}}(f)\define \inf\{\rho \in \real_{\geq 0}: \rho^{-1}f \in \mathfrak{F}\}\label{eq:minkowski-functional}$, this implies that for any function $f$: $\vert\int_{\mathcal{E}}fd\nu_1 - \int_{\mathcal{E}}fd\nu_2 \vert\leq \rho_{\mathfrak{F}}(f)\ipm(\nu_1,\nu_2) \label{eq:ipm-implication}$. 
    
    Consider a history-based feature map that is recursively updatable \ie, there exists an update function $\hat f$ such that $\Ais_{\timestep+1} = \hat f (\Ais_\timestep, \Action_\timestep, \State_{\timestep+1})$. Given such a recursively-updatable history based feature map and an $(\epsilon, \delta)$ AIS generator $(\hat \cost, \hat \transition)$, define the following dynamic program: 
    
    \begin{equation}
                \hat Q(\ais, \action) = \hat \cost(\ais, \action) + \discount \sum_{\sts \in \statespace}
                \hat \transition(\sts|\ais,\action) \hat \valuefunction(\hat{f}(\ais,\sts,\action)), \ \forall \feature \in \featurespace, \action \in \actionspace \qquad
                \hat \valuefunction(\ais) = \max_{\action \in \actionspace} \hat Q(\ais,\action), \ \forall \feature \in \featurespace \label{eq:ais-dp}
    \end{equation}
    
    Now, let $\mu \colon \aisspace \to \Delta(\actionspace)$ be any policy such that for any $\ais \in \aisspace$, $\support(\mu(\ais)) \subseteq \arg\max_{\action \in \actionspace} \hat Q(\ais,\action)\label{eq:policy}$.
    Note that $\mu$ is a policy from the feature space to actions, and we can use it to define a policy from the history of the state action pairs to actions as: $\policy{}_{\timestep}(\sts_{1:\timestep}, \action_{1:\timestep-1}) = \mu(\aisfunction_{\timestep}(\sts_{1:\timestep}, \action_{1:\timestep-1}))$, which then implies that $\policy{} = \{\policy{}_\timestep\}_{\timestep \geq 1}$ is a history-based policy. Thus the dynamic program defined in \eqref{eq:ais-dp} indirectly defines a history-based policy $\policy{}$. We provide the following bound on the performance of $\policy{}$ and the optimal (state-based) policy $\policy^*$. 
    %A natural question which then arises is that \emph{how can we bound the sub-optimality gap between $\policy^\star$ and $\policy{}$?} We answer this question in the following result:
    \begin{theorem}\label{thm:ais-dp}
      For any time $\timestep$, any realisation $\sts_\timestep$ of $\State_\timestep$, $\action_\timestep$ of $\Action_\timestep$, let $\history_\timestep = (\sts_{1:\timestep}, \action_{1:\timestep-1})$, and $\ais_\timestep = \aisfunction_\timestep(\history_\timestep)$. Additionally, let $\valuefunction^{\policy{}}$ be the value of using the history-based policy $\policy{}$ as defined in \eqref{eq:policy} to control the MDP $\mdp$.
      Define the worst case difference between $\valuefunction^{\star}$ and $\valuefunction^{\policy{}}$ as, $   \Delta = \sup_{\timestep \geq 0}\sup_{\history_\timestep = (\sts_{1:\timestep}, \action_{1:\timestep}) \in \historyspace_\timestep} \vert \valuefunction^{\star}(\sts_\timestep) - 
      \valuefunction^{\policy{}}(\ais_\timestep)\vert$.
      Then 
      \begin{equation}
        \Delta
        \le 2 \frac{\varepsilon + \discount\delta \kappa_{\mathfrak{F}}(\hat \valuefunction^{\mu}, \hat{f})}{1 - \discount},\label{eq:ais-bound}
      \end{equation}
      where, $\kappa_{\mathfrak{F}}(\hat \valuefunction^\mu, \hat f)$ 
      is a quantity that depends on the choice of the IPM $d_{\mathfrak{F}}$. 
    \end{theorem}

    We can further show the following.
    (a)~When $\ipm$ is the total variation distance, then 
        $\kappa_{\mathfrak{F}}(\hat \valuefunction^\mu, \hat f) = \spn(\hat \cost)/(1-\discount)$. 
    (b)~When $\ipm$ is the Wasserstein distance, then
    $\kappa_{\mathfrak{F}}(\hat \valuefunction^\mu, \hat f) = L_{\hat \cost}/(1-\discount L_{\hat f} L_{\hat \transition})$, where for any function~$f$, $L_f$ denotes its Lipschitz constant.  
    (c)~When $\ipm$ is the Maximum Mean Discrepancy (MMD) distance, 
    $\kappa_{\mathfrak{F}}(\hat \valuefunction^{\mu}, \hat{f})  = \sup_{\feature, \action}\Vert(\hat \valuefunction(\hat f(\cdot, \feature, \action)))\Vert_{\mathcal{U}}$, where $\| \cdot \|_{\mathcal{U}}$ is the RKHS norm.
    
    %If $\ipm$ is the Kantorovich-Rubinstein/Wasserstein distance, then its Minkowski functional is $\rho_{\mathfrak{F}^W}(f) = L_f$ where $L_f$ denotes the Lipschitz constant of any function $f$ with respect to the metric on $\mathcal{E}$, and $\kappa_{\mathfrak{F}}(\hat \valuefunction^{\mu}, \hat{f}) = L_{\hat \cost}/1 - \discount L_{\hat f}L_{\hat \transition}$. Finally, if $\ipm$ is the Maximum Mean Discrepancy (MMD) distance, then its Minkowski functional is $\rho_{\mathfrak{F}^{\text{MMD}}}(f) = \Vert f\Vert _{\mathcal{U}}$, where for any function $f$, $\Vert \cdot \Vert_{\mathcal{U}}$ denotes the RKHS norm, and $\kappa_{\mathfrak{F}}(\hat \valuefunction^{\mu}, \hat{f})  = \sup_{\feature, \action}\Vert(\hat \valuefunction(\hat f(\cdot, \feature, \action)))\Vert_{\mathcal{U}}$.
    
    The above results bound the worst case performance loss of the best feature-based policy given a particular AIS generator. The loss function can be used as an auxiliary loss to optimise the AIS generator. In the next section, we build on this idea to construct an RL algorithm.
    
       
         \begin{corollary}\label{THM:TV-BOUND}
             If the function class $\mathfrak{F}$ is $\mathfrak{F}^{\text{TV}}$, then $\Delta$ as defined in  \Cref{thm:ais-dp} is upper bounded as:
             \begin{align}
              \Delta
                \le  \frac{2\epsilon}{(1-\discount)} +  \frac{\discount\delta \spn(\hat\cost)} {(1-\discount)^2},
            \end{align}
        \end{corollary}
        
            Proof in Appendix \ref{sec:tv-proof}
        
        \begin{corollary}\label{THM:LIP-BOUND}
            If $\discount L_{\hat \transition}L_{\hat f} \leq 1$ and the function class $\mathfrak{F}$ is $\mathfrak{F}^{\text{W}}$, then $\Delta$ as defined in  \Cref{thm:ais-dp} is upper bounded as:
            \begin{align}
                \Delta
                \le  \frac{2\epsilon}{(1-\discount)} + \frac{2\discount\delta L_{\hat \cost} }{(1- \discount)(1-\discount L_{\hat f}L_{\hat\transition})},
            \end{align}
        \end{corollary}
        where $L_{\hat \cost}$ and $L_{\hat{\transition}}$ are the Lipschitz constants of the approximate reward function $\hat \cost$ and approximate transition function $\hat \transition$ respectively, and $L_{\hat f}$ is the uniform bound on the Lipschitz constant of $\hat f$ with respect to the state $\State_\timestep$.

            Proof in Appendix \ref{sec:w-proof}

        \begin{corollary}\label{thm:mmd-bound}
             If the function class $\mathfrak{F}$ is $\mathfrak{F}^{\text{MMD}}$, then $\Delta$ as defined in  \Cref{thm:ais-dp} is upper bounded as:
             \begin{align}
              \Delta
                \le  2 \frac{\epsilon + \discount\delta\kappa_{\mathcal{U}}(\hat \valuefunction, \hat f) } {(1-\discount)},
            \end{align}
            where similar to \Cref{def:mmd-dist}, $\mathcal{U}$ is a RKHS space,  $\Vert\cdot\Vert_{\mathcal{U}}$ its associated norm and $\kappa_{\mathcal{U}}(\hat \valuefunction, \hat f) = \sup_{\feature, \action}\Vert(\hat \valuefunction(\hat f(\cdot, \feature, \action)))\Vert_{\mathcal{U}}$.
        \end{corollary}
        \begin{proof}
            The proof follows in a straight forward way from the properties of MMD described previously. 
        \end{proof}
    
   


==> sections/model.tex <==
\section{Background and Motivation}\label{sec:background}
        \begin{figure*}[!ht]
          \centering
          \begin{minipage}{0.75\linewidth}
          \subfigure[$P(0)$]{
            \begin{tikzpicture}[thick,scale=0.65]
              \node [agent] at (0, 0) (0) {$0$};
              \node [agent] at (1, 0) (1) {$1$}; 
              \node [agent] at (0, 1) (3) {$3$};
              \node [agent] at (1, 1) (2) {$2$};
              \path[->]
                    (0) edge node[below] {$0.5$} (1)
                    (1) edge node[right] {$0.5$} (2)
                    (2) edge node[above] {$0.5$} (3)
                    (3) edge node[left]  {$0.5$} (0)
                    (0) edge[loop left] node {$0.5$} (0)
                    (1) edge[loop right] node {$0.5$} (1)
                    (2) edge[loop right] node {$0.5$} (2)
                    (3) edge[loop left] node {$0.5$} (3)
                    ;
            \end{tikzpicture}}
           \hfill
          \subfigure[$P(1)$]{
            \centering
            \begin{tikzpicture}[thick,scale=0.75]
              \node [agent] at (0, 0) (0) {$0$};
              \node [agent] at (1, 0) (1) {$1$}; 
              \node [agent] at (0, 1) (3) {$3$};
              \node [agent] at (1, 1) (2) {$2$};
              \path[<-]
                    (0) edge node[below] {$0.5$} (1)
                    (1) edge node[right] {$0.5$} (2)
                    (2) edge node[above] {$0.5$} (3)
                    (3) edge node[left]  {$0.5$} (0)
                    (0) edge[loop left] node {$0.5$} (0)
                    (1) edge[loop right] node {$0.5$} (1)
                    (2) edge[loop right] node {$0.5$} (2)
                    (3) edge[loop left] node {$0.5$} (3)
                    ;
            \end{tikzpicture}}
            \hfill
            \subfigure[$P(2)$]{%
                  \begin{tikzpicture}[thick,scale=0.65]
                  \node [agent] at (0, 0) (0) {$0$};
                  \node [agent] at (1, 0) (1) {$1$}; 
                  \node [agent] at (0, 1) (3) {$3$};
                  \node [agent] at (1, 1) (2) {$2$};
                  \path[->]
                        (0) edge [bend right] node[below] {$0.5$} (1)
                        (1) edge [bend right] node[right] {$0.5$} (2)
                        (2) edge [bend right] node[above] {$0.5$} (3)
                        (3) edge [bend right] node[left]  {$0.5$} (0)
                        (0) edge [bend right] node[right] {} (3)
                        (3) edge [bend right] node[below] {} (2)
                        (2) edge [bend right] node[left]  {} (1)
                        (1) edge [bend right] node[above]  {} (0);
                \end{tikzpicture}}
                \caption{The transition probability model for the example of}
          \label{fig:P}
          \end{minipage}%
          \begin{minipage}{0.25\linewidth}
          \centering
            \begin{tikzpicture}[thick,scale=0.9]
              \node [agent] at (0, 0) (0) {$0$};
              \node [agent] at (1, 0) (1) {$1$}; 
              \node [agent] at (0, 1) (3) {$3$};
              \node [agent] at (1, 1) (2) {$2$};
              \path[->]
                    (0) edge node[below] {$0.5$} (1)
                    (1) edge[bend right] node[right] {$0.5$} (2)
                    (2) edge[bend right]  node[left] {$0.5$} (1)
                    (3) edge node[left]  {$0.5$} (0)
                    (3) edge node[above] {$0.5$} (2)
                    (0) edge[loop left] node {$0.5$} (0)
                    (1) edge[loop right] node {$0.5$} (1)
                    (2) edge[loop right] node {$0.5$} (2)
                    (3) edge[loop left] node {$0.5$} (3)
                    ;
            \end{tikzpicture}
          \caption{The transition probability of the optimal policy}
          \label{fig:optimal}
          \end{minipage}
        \end{figure*}

    % \subsection{Function approximation in MDPs}
    
        Consider an MDP $ \mdp = \langle \statespace, \actionspace, \transition, \cost, \discount \rangle$ where $\statespace$ denotes the state space, $\actionspace$ denotes the action space, $\transition$ denotes the controlled transition matrix, $\cost \colon \statespace \times \actionspace \to \real$ denotes the per-step reward, and $\discount \in (0,1)$ denotes the discount factor.
                
        The performance of a randomised (and possibly history-dependent) policy $\policy$
        starting from a start state $\sts_{0}$ is measured by the value function, defined as:
        \begin{equation}
          \valuefunction^{\policy}(\sts_0) = \expecun{}^{\policy}\bigg[\sum_{\timestep=0}^{\infty}\discount^{\timestep}\cost(\State_{\timestep},\Action_{\timestep}) \bigg| \State_{0} = \sts_{0}\bigg].
        \end{equation}
        A policy maximising $\valuefunction^{\policy}(\sts_0)$ over all (randomized and possibly history dependent) policies is called the optimal policy with respect to initial state $s_0$ and is denoted by $\policy^{\star}$\footnote{This notion can easily be extended to start state distributions.}.
                
        In many applications, $\statespace$ and $\actionspace$ are combinatorially large or uncountable, which makes it intractable to compute the optimal policy. 
        Most practical RL algorithms overcome this hurdle by using function approximation where the state is mapped to a feature space $\featurespace$ using a state abstraction function $\basis:\statespace \to \featurespace$. In Deep-RL algorithms, the last layer of the network is often viewed as a feature vector. These feature vectors are then used as an approximate state for approximating the value function $\hat\valuefunction: \featurespace \to \real$ and/or computing an approximately optimal policy $\mu:\featurespace \to \Delta(\actionspace)$~\citep{Sutton+Barto:1998} (where $\Delta(\actionspace)$ denotes the set of probability distribution over actions). We use $\tilde{\mu} = \mu \circ \basis$ ~\ie, $\tilde{\mu} = \mu(\phi(\cdot))$ to denote the ``flattened" policy that maps states to action distributions.
        
        % The features $\Feature_\timestep$ are then used as an approximate state for computing the value function $\hat\valuefunction: \featurespace \to \real$ and/or the policy $\mu:\featurespace \to \Delta(\actionspace)$~\citep{Sutton+Barto:1998} (where $\Delta(\actionspace)$ denotes the set of probability distribution over actions). We denote by $\mu \circ \phi $ as the ``flattened" policy that maps states to action distributions, by composing the feature abstraction and the policy acting on it. In Deep-RL algorithms, the output of the last layer of the network is often viewed as the feature vector $\Feature_{\timestep}$.
        
        % A well known yet often overlooked fact about function approximation is that the features used as a proxy state may not satisfy the controlled Markov property \ie, in general,
        A well known fact about function approximation is that the features that are used as an approximate state may not satisfy the controlled Markov property \ie, in general, 
        \[
            \prob(\Feature_{\timestep+1} \mid \Feature_{1:\timestep}, \Action_{1:\timestep}) \neq
            \prob(\Feature_{\timestep+1} \mid \Feature_\timestep, \Action_\timestep).
        \]

        To see the implications of this fact, consider the toy MDP depicted in Fig.~\ref{fig:P}, with $ \statespace = \{0, 1, 2, 3\}$, $\actionspace =
        \{0, 1, 2\}$, $\{\transition_{\sts, \sts'}(\action)\}_{\action \in \actionspace}$, and $r(0) = r(1) = -1$, $r(2) = 1$, $r(3) = -K$, where $K$ is a large positive number.
       Given the reward structure the objective of the policy is to try to avoid state~$3$ and keep the agent at state~$2$ as much as possible. It is easy to see that the optimal policy is 
            \[
              \pi^\star(0) = 0, \quad
              \pi^\star(1) = 0, \quad
              \pi^\star(2) = 1,
              \text{ and}\quad
              \pi^\star(3) = 2.
            \]
        The Markov chain induced by the optimal policy is shown in Fig.~\ref{fig:optimal}. 
        Note that if the initial state is not state~$3$ then an agent will never visit that state under the optimal policy. Furthermore, any policy which cannot prevent the agent from visiting state~$3$ will have a large negative value and, therefore, cannot be optimal.
        Now suppose the feature space $\featurespace = \{0, 1\}$. It is easy to see that for any Markovian feature-abstraction $\policyencoder{} \colon \statespace \to \featurespace$, no policy $\hat \pi \colon \featurespace \to \actionspace$ can prevent the agent from visiting state~$3$. Thus, the best policy when using Markovian feature abstraction will perform significantly worse than the optimal policy (which has direct access to the state).
    
        However, it is possible to construct a history-based feature-abstraction  $\policyencoder$ and a history-based control policy $\hat \pi$ that works with $\phi$ and is of the same quality as $\pi^\star$. For this, consider the following \emph{codebooks} (where the entries denoted by a dot do not matter):
        \begin{align*}
          F(1) &= \begin{bmatrix}
            0 & 1 & \cdot & \cdot \\
            \cdot & 0 & 1 & \cdot \\
            \cdot & \cdot & 0 & 1 \\
            1 & \cdot & \cdot & 0
          \end{bmatrix}, 
          &
          F(2) &= \begin{bmatrix}
            1 & \cdot & \cdot & 0 \\
            0 & 1 & \cdot & \cdot \\
            \cdot & 0 & 1 & \cdot \\
            \cdot & \cdot & 0 & 1
          \end{bmatrix} ,
           \\
          F(3) &= \begin{bmatrix}
            \cdot & 0 & \cdot & 1 \\
            0 & \cdot & 1 & \cdot \\
            \cdot & 0 & \cdot & 1 \\
            0 & \cdot & 1 & \cdot
          \end{bmatrix},
          &
          D(0) &= \begin{bmatrix}
            0 & 1 \\
            1 & 2 \\
            2 & 3 \\
            3 & 0 
          \end{bmatrix} ,
          \\
          D(1) &= \begin{bmatrix}
            3 & 0 \\
            0 & 1 \\
            1 & 2 \\
            2 & 3 
          \end{bmatrix} ,
          &
          D(2) &= \begin{bmatrix}
            1 & 3 \\
            0 & 2 \\
            1 & 3 \\
            0 & 2 
          \end{bmatrix} .
        \end{align*}
        Now consider the following feature-abstraction:
        \[
          Z_t =  F_{S_{t-1}, S_t}(A_{t-1}),
        \]
        and a control policy $\mu$ which is a finite state machine with memory $M_t$ that is updated as:
        \[
          M_t = D_{M_{t-1}, Z_t}(A_{t-1})
        \]
        and chooses the actions according to:
        \[
          \quad
          A_t = \pi(M_t),
        \]
        where $\pi \colon \statespace \to \Delta(\actionspace)$ is any pre-specified reference policy. It can be verified that if the system starts from a known initial state then $\mu \circ \basis = \pi$. 
         Thus, if we choose the reference policy $\pi=\pi^\star$, then
        the agent will never visit state~$3$ under $\mu \circ \basis$, in contrast to Markovian feature-abstraction policies where (as we argued before) state~$3$ is always visited.
        
        From the above example, we can see that when system dynamics are known, one can exploit the problem structure to design history-based feature abstractions which outperform their memoryless counterparts. However, such constructions are not feasible in the general learning setup, where the system dynamics are unknown. 
        % One way to overcome this issue is to let the policy $\policy{}$ be a function of all the information available to the system at time $\timestep$  ~\ie, $\policy{}_\timestep: \historyspace_{\timestep} \to \Delta(\actionspace)$ where, $\historyspace_\timestep \define \{\statespace^{1:\timestep},\featurespace^{1:\timestep-1}, \actionspace^{1:\timestep-1}\}$. 
        We can overcome this issue by letting the policy be a function of the history of state, actions and observations observed until time $\timestep$, \ie, $\policy{}_\timestep: \historyspace_{\timestep} \to \Delta(\actionspace)$ where, $\historyspace_\timestep \define \{\statespace^{1:\timestep},\featurespace^{1:\timestep-1}, \actionspace^{1:\timestep-1}\}$. 
        
        % Since the environment is an MDP, the state $\State_\timestep$ is  a sufficient statistic and the loss of information happens when $\State_\timestep$ is mapped to $\Feature_\timestep$. This is a subtle yet critical distinction between POMDPs and function approximation in MDPs. In POMDPs the state signal is unavailable, and the system only sees a observation vector $\Feature_\timestep$. Whereas, in function approximation setup, we can observe the state signal perfectly and partial observability is induced due to feature abstraction. Therefore, we can discard the the history of states and focus on the policies of the following form $\policy{}_\timestep: \historyspace_{\timestep} \to \Delta(\actionspace)$ where, $\historyspace_\timestep \define \{\statespace,\featurespace^{1:\timestep-1}, \actionspace^{1:\timestep-1}\}$.   
        
        As the size of history grows with time $t$ and it is computationally and conceptually difficult to use it for deriving a dynamic programming decomposition. One solution is to map the history to a fixed dimensional representation and use it as a state for designing a dynamic program. One can think of such a representation as an information state.  Due to lossy compression a prefect information state may be hard to obtain, but we an construct an approximate information state (AIS) such that it satisfies the controlled Markov property and captures the sufficient information for identifying the policy. In the next section we will show how to construct and AIS and use it for obtaining a dynamic program, which can then be solved, either exactly or approximately, to obtain a policy with a bounded approximation error. 
        
        % One can think of this representation as an information state ~\citep{kwakernaakh.1965,infostate-Witsenhausen,Striebel1965SufficientSI,Bohlin1970InformationPF,Davis1972InformationSF,Kumar1986StochasticSE}. 
        
        
    \section{Main Results}\label{sec:main}
    
        As mentioned previously, we can use the history of state, action and observations to learn the feature abstractions, but it possible to simplify this information structure further. Note that, as the environment is an MDP, the state $\State_\timestep$ is a sufficient statistic. The loss of information happens when $\State_\timestep$ is mapped to $\Feature_\timestep$. This is a subtle yet critical distinction between POMDPs and function approximation in MDPs. In POMDPs the state signal is unavailable, and the system only sees a observation vector $\Feature_\timestep$. Whereas, in function approximation setup, we can observe the state signal perfectly and partial observability is induced due to feature abstraction. Therefore, we can discard the the history of states and focus on the policies of the following form $\policy{}_\timestep: \historyspace_{\timestep} \to \Delta(\actionspace)$ where, $\historyspace_\timestep \define \{\statespace,\featurespace^{1:\timestep-1}, \actionspace^{1:\timestep-1}\}$. Despite this simplification the size of history is growing with time and history compression is still required. As such, we will now proceed towards defining the AIS for MDPs to address all of the aforementioned issues. 

      Given an MDP $\mdp$ and a feature space $\aisspace$, let $\historyspace_t = \statespace \times \featurespace^{\timestep-1} \times \actionspace^{\timestep-1}$ denote the space of all histories $(\State_\timestep, \Feature_{1:t}, \Action_{1:t-1})$ up to time~$t$. We are interested in learning history-based feature abstraction functions $\{ \aisfunction_t \colon \historyspace_t \to \aisspace \}_{t \ge 1}$ and a policy $\mu \colon \aisspace \to \Delta(\actionspace)$ such that $\policy{} = \{\policy{}_\timestep\}_{\timestep \ge 1}$, where $\policy{}_\timestep = \mu \circ \aisfunction_\timestep$, is approximately optimal. 

        
        Before defining the main model we will start with some necessary technical definitions.
        
        \subsection{Integral probability metrics (IPM)}
            \begin{definition}[~\citep{ipm}]
                    Let $(\mathcal{E},\mathcal{G})$ be a measurable space and $\mathfrak{F}$ denote a class of uniformly bounded measurable functions on $(\mathcal{E},\mathcal{G})$. The integral probability metric between two probability distributions  $\nu_1, \nu_2 \in \mathcal{P}(\mathcal{E})$ with respect to the function class $\mathfrak{F}$ is defined as:
                    \begin{align}
                        \ipm(\nu_1, \nu_2) &= \sup_{f \in \mathfrak{F}}\bigg| \int_{\mathcal{E}}f d\nu_1  - \int_{\mathcal{E}}f d\nu_2\bigg|.\label{eq:def-ipm}
                    \end{align}
                    
                    For any function $f$ (not necessarily in $\mathfrak{F}$), the Minkowski functional $\rho_{\mathfrak{F}}$ associated with the $\ipm$ is given as:
                    \begin{align}
                        \rho_{\mathfrak{F}}(f)&\define \inf\{\rho \in \real_{+}: \rho^{-1}f \in \mathfrak{F}\}.\label{eq:minkowski-functional}
                    \end{align}
                    
                    \Cref{eq:minkowski-functional}, implies that that for any function $f$:
                    \begin{align}
                         \bigg|\int_{\mathcal{E}}fd\nu_1 - \int_{\mathcal{E}}fd\nu_2 \bigg|\leq \rho_{\mathfrak{F}}(f)\ipm(\nu_1,\nu_2) \label{eq:ipm-implication}
                     \end{align}
                    
            \end{definition}
            
            \noindent Some examples of IPMs are:
            \begin{example}\label{def:tv-dist}
                If $\mathfrak{F}$ is chosen as $\mathfrak{F}^{\text{TV}}\define \{\frac{1}{2}\spn(f) = \frac{1}{2}(\max(f)- \min(f))\}$, then $\ipm$ is the total variation distance, and its Minkowski functional is: $\rho_{\mathfrak{F}}(f) = \frac{1}{2}\spn(f)$. 
            \end{example}
            \begin{example}\label{def:kr-dist}
                 If $\mathcal{E}$ is a metric space and $\mathfrak{F}$ is chosen as $\mathfrak{F}^{W} \define \{f: L_f \leq 1 \}$(where $L_f$ denotes the Lipschitz constant of $f$ with respect to the metric on $\mathcal{E}$), then $\ipm$ is the Wasserstein or the Kantorovich distance. The Minkowski function for the Wasserstein distance is a $\rho_{\mathfrak{F}^W}(f) = L_f$
            \end{example}
            
            \begin{example}\label{def:mmd-dist}
                Let $\mathcal{U}$ be a reproducing kernel Hilbert space (RKHS) of real-valued functions on $\mathcal{E}$ and $\mathfrak{F}$ is choosen as $\mathfrak{F}^{MMD} \define \{f\in \mathcal{U}: \Vert f \Vert _{\mathcal{U}} \leq 1 \}$, (where $\Vert \cdot \Vert_{\mathcal{U}}$ denotes the RKHS norm), then $\ipm$ is the Maximum Mean Discrepancy (MMD) distance and its Minkowski functional is $\rho_{\mathfrak{F}^{\text{MMD}}}(f) = \Vert f\Vert _{\mathcal{U}}$

            \end{example}
 
            
        \subsection{Approximate information state}
        
        \begin{definition}\label{def:state-update}
                A family of history-based feature abstraction functions  $\{\aisfunction_\timestep: \historyspace^{\timestep} \to \featurespace\}_{\timestep \geq 1}$ are said to update recursively if there exists an function $\hat f: \featurespace \times \statespace \times \actionspace \to \featurespace $ such that the process $\{\Feature_\timestep\}_{\timestep\geq 1}$ satisfies:
                \begin{align}
                    \Feature_{\timestep +1} = \hat f(\Feature_\timestep, \State_\timestep, \Action_\timestep),
                \end{align}
                where, $\Feature_\timestep = \aisfunction_\timestep(\State_{\timestep}, \Feature_{1:\timestep-1} \Action_{1:\timestep-1})$.
        \end{definition}
        
        \begin{definition}\label{def:ais}
            Given a family of history based feature abstraction functions $\{\aisfunction_\timestep: \historyspace^{\timestep} \to \featurespace\}_{\timestep \geq 1}$, the features $\Feature_\timestep = \aisfunction(\State_{\timestep}, \Feature_{1:\timestep-1}, \Action_{1:\timestep-1})$ are said to be $(\epsilon, \delta)$-Approximate information state with respect to a function space $f$, if there exist: 
            \begin{itemize}
                \item Reward approximation function: $\hat r: \featurespace \times \actionspace \to \real$
                \item Approximate Transition kernel: $\hat\transition: \featurespace \times \actionspace \to \Delta(\statespace)$
            \end{itemize}
            The tuple $(\hat r ,\hat\transition)$ is called an $(\epsilon, \delta)$- AIS approximator if the AIS satisfies the following properties:
            
            \begin{property}\label{p1}
                \textbf{\textit{Sufficient for approximate performance evaluation:}}
                \begin{align}
                  \forall \timestep \, \  | \cost(\State_{\timestep}, \Action_{\timestep})
                                            - \hat{\cost}(\Feature_\timestep, \Action_\timestep)| \leq \epsilon.
                 \label{def:p1}
                \end{align}
            \end{property}
            \begin{property} \label{p2b}
            \textbf{\textit{Is sufficient for predicting future states approximately:}} 
            \begin{align}
                \forall \timestep \ , \ d_{\mathfrak{F}}(\transition(\cdot \vert \State_\timestep, \Action_\timestep), \hat \transition(\cdot\vert \Feature_\timestep, \Action_\timestep)) &\leq \delta_{d_{\mathfrak{F}}}.
                % \text{with }\kappa_{\ipm}(\hat{f}_\timestep) &\define \sup_{\history_\timestep, \action_\timestep} \bigg[ \kappa_{\ipm}(\hat{f}_\timestep (\aisfunction_\timestep (\history_\timestep), \cdot, \action_\timestep))\bigg].
            \end{align}
        \end{property}
            
        \end{definition}
        \Cref{def:state-update}, \Cref{p1,p2b} help us ensure that the history compression (approximately) satisfies the properties of state so that we can use it for designing dynamic program as follows:
        % \subsubsection{AIS based dynamic program}
        \begin{theorem}\label{thm:ais-dp}
            Given an $(\epsilon, \delta)$ AIS approximator $(\hat \transition, \hat \cost)$, and history-based abstraction functions $\{\aisfunction_\timestep: \historyspace^\timestep \to \featurespace\}_{\timestep \geq 1}$ that update as per $\hat f$, define the following: 
            % Given a state-update function $\hat{f}$ and an AIS generator $\{\aisfunction_\timestep, \hat \transition_\timestep, \hat \cost_\timestep\}_{\timestep = 1}^{\infty}$, where $\aisfunction_\timestep$ is defined based on $\hat{f}$, define the following:
            
            \begin{align}
                \hat Q(\ais, \action) &= \hat \cost(\ais, \action) + \discount \sum_{\sts \in \statespace}
                \hat \transition(\sts|\ais,\action) \hat \valuefunction(\hat{f}(\ais,\sts,\action)), \\
                \hat \valuefunction(\ais) &= \max_{\action \in \actionspace} \hat Q(\ais,\action),\label{eq:ais-dp}
            \end{align}
            and let $\mu \colon \aisspace \to \Delta(\actionspace)$ be any policy such that for any $\ais \in \aisspace$,
            \[
                \text{Supp}(\mu(\ais)) \subseteq 
                \arg\max_{\action \in \actionspace} \hat Q(\ais,\action).
            \]
            Define the policy $\policy{} = \{\policy_\timestep\}_{\timestep = 1}^{\infty}$ where $\policy_\timestep = \mu \circ \aisfunction_\timestep$. Then, loss of performance incurred by $\policy{}$ is bounded as follows:
            \begin{align}
                \valuefunction^{\policy{}^\star}(\sts_0) - \hat{\valuefunction}^{\policy{}}(\feature_0)
                \le \frac{\varepsilon + \discount\delta_{d_{\mathfrak{F}}} \rho_{\mathfrak{F}}( \hat\valuefunction^{\policy{}}) \kappa_{\mathfrak{F}}(\hat{f})}{1 - \discount},\label{eq:ais-bound}
            \end{align}

            where $\kappa_{\mathfrak{F}}(\hat{f}) \define \sup_{\history_\timestep, \action_\timestep} \bigg[ \rho_{\mathfrak{F}}(\hat{f} (\aisfunction_\timestep (\history_\timestep), \cdot, \action_\timestep))\bigg]$.
        \end{theorem}
        Proof in \Cref{sec:proof:thm:ais-dp}
        
        
        {\color{blue}{Proof and Remarks to be discussed with Aditya.}}
        
        In \eqref{eq:ais-bound}, $\epsilon$ and $\delta$, capture the worst case error incurred by the AIS when predicting instantaneous reward $\cost$ and approximating the transition distribution of the ground MDP $\mdp$. Therefore, resulting suboptimality bound helps us quantify us the loss in performance due to feature abstraction. At the same time, the IPM used for measuring the distance between the approximate and true transition distribution also influences the bound via $\rho_{\mathfrak{F}}(\hat\valuefunction)$ and $\kappa_{\mathfrak{F}}(\hat f)$. In the following corollaries we will show how $\rho_{\mathfrak{F}}$ and $\kappa_{\mathfrak{F}}(\hat f)$ take specific forms according the choice of the IPM.
        
         \begin{corollary}\label{thm:tv-bound}
             If the function class $\mathfrak{F}$ is $\mathfrak{F}^{\text{TV}}$, then the result in \Cref{thm:ais-dp} is:
             \begin{align}
                \valuefunction^{\policy{}^\star}(\sts_0) - \hat{\valuefunction}^{\policy{}}(\feature_0)
                \le  \frac{\epsilon + \discount\delta \spn(\hat\valuefunction) \spn(\hat f)} {(1-\discount)},
            \end{align}
        \end{corollary}
        
        
        \begin{corollary}\label{thm:lip-bound}
            If the function class $\mathfrak{F}$ is $\mathfrak{F}^{\text{W}}$, then the result in \Cref{thm:ais-dp} is:
            \begin{align}
                \valuefunction^{\policy{}^\star}(\sts_0) - \hat{\valuefunction}^{\policy{}}(\feature_0)
                \le  \frac{\epsilon + \discount\delta L_{\hat\valuefunction} L_{\hat{f}}}{(1-\discount)},
            \end{align}
            where $L_{\hat\valuefunction}$ and $L_{\hat{f}}$ denote the Lipschitz constants of $\hat V$ and $\hat f$ respectively.
        \end{corollary}
        
        \begin{corollary}\label{thm:mmd-bound}
             If the function class $\mathfrak{F}$ is $\mathfrak{F}^{\text{MMD}}$, then the result in \Cref{thm:ais-dp} is:
             \begin{align}
                \valuefunction^{\policy{}^\star}(\sts_0) - \hat{\valuefunction}^{\policy{}}(\feature_0)
                \le  \frac{\epsilon + \discount\delta \Vert\hat\valuefunction \Vert_{\mathcal{U}} \Vert \hat{f} \Vert_{\mathcal{U}}} {(1-\discount)},
            \end{align}
            where similar to \Cref{def:mmd-dist}, $\mathcal{U}$ is a RKHS space and  $\Vert\cdot\Vert_{\mathcal{U}}$ is the norm associated with it.
        \end{corollary}
        
        Additionally, all the constants in \eqref{eq:ais-bound} are influenced by how one constructs and obtains an AIS. Since the an AIS is primarily a compression of history, we can learn it using a carefully designed data-driven algorithm. Such as AIS can then be used for approximately solving dynamic program in \eqref{eq:ais-dp} using RL.
        In the following section we will show how one can design a multi-timescale RL algorithm for simultaneously learning the AIS and policy $\policy{}$.

==> sections/results.tex <==
    \begin{figure}[!htbp]
      \includegraphics[width=\linewidth]{Results/combined-1.pdf}
      % \caption{This is a figure} \label{fig:comb-results-1}
      \includegraphics[width=\linewidth]{Results/combined-2.pdf}
      \caption{PPO using feed-forward NN, GRU and AIS, averaged over 50 Monte Carlo runs with $\pm$1 \texttt{std-dev}.} \label{fig:comb-results-2}
    \end{figure}
\section{Empirical evaluation}\label{sec:experiments}

    Through our experiments, we seek to answer the following questions:
    (1) Can history-based feature representations policies help improve the quality of solution found by a memory-less RL algorithms?
    (2) In terms of the solution quality how does the proposed method compare with other methods which use memory augmented policies as well as reward and transition predictors?
    (3) How does the choice of IPM affect the algorithms performance?

    % Through our experiments, we seek to answer the following questions:
    % (1) Can history-based feature representation policies help improve the quality solution found by a memory-less RL algorithm?
    % (2) In regards to the solution quality and sample complexity, how does the proposed method compare with other memory-augmented policies?
    % (3) How does the choice of IPM affect the algorithms performance?
    
    We answer question (1) and (2) by comparing our approach with the proximal policy gradient (PPO) algorithm which uses feed-forward neural networks. For question (2), we compare our method with an LSTM-based PPO variant which learns the feature representation using the history of states $\State_{1:\Timestep}$ in a trajectory. For question (3) we compare the performance of our method using different MMD kernels and KL-divergence based approximation of Wasserstein distance. All the approaches are evaluated on six continuous control tasks from the MuJoCo~\citep{Todorov2012MuJoCoAP} OpenAI-Gym suite. To ensure a fair comparison, the baselines and their respective hyper-parameter settings are taken from well tested stand-alone implementations provided by~\citet{baselines}. From an implementation perspective, our framework can be used to modify any off-the-shelf policy-gradient algorithm by simply replacing (or augmenting) the feature abstraction layers of the policy and/or value networks with recurrent neural networks (RNNs), trained with the appropriate losses, as outlined previously. In these experiments, we replace the fully connected layers in PPO's architecture with a Gated Recurrent Unit (GRU). For all the implementations, we initialise the hidden state of the GRU to zero at the beginning of the trajectory. This strategy simplifies the implementation and also allows for independent decorrelated sampling of sequences, therefore ensuring robust optimisation of the networks~\citep{rnn-hausknecht}. It is important to note that we can extend our framework to other policy gradient methods such as SAC~\citep{HaarnojaZAL18}, TD3~\citep{td3} or DDPG~\citep{ddpg}, after satisfying certain technical conditions. However, we leave these extensions for future work. Additional experimental details and results can be found in \Cref{sec:experiment-details}.
    
    
%\subsection{Numerical Results} 
    
     \Cref{fig:comb-results-2} contains the results of our experiments averaged over 50 Monte-Carlo evaluations using MMD-based AIS loss in \eqref{eq:mmd-ais-loss}.  These results show that our algorithm improves over the performance of both the baselines, and the performance gain is significantly higher for high-dimensional environments like Humanoid and Ant. 
     It is worth noticing that the GRU baseline also outperforms the feed-forward baseline for most  environments. Overall, these findings lend credence to  history-based encoding policies as a way to improve the quality of the solution learnt by the RL algorithm.
    % \begin{table}
    %     \resizebox{\columnwidth}{!}
    %     {
    %      \begin{tabular}{||c |c| c| c |c ||} 
    %      \hline
    %      Environment & PPO(1e3) & PPO-RNN(1e3) & Ciac-a(1e3) & Ciac-b(1e3) \\ [0.3ex] 
    %      \hline\hline
    %      Half-Cheetah & 1.64$\pm$0.74 & 2.91$\pm$1.13 & 5.16$\pm$0.47 & 4.30$\pm$0.38 \\ 
    %      \hline
    %      Ant & 3.36$\pm$0.18 & 4.16$\pm$ 0.14 & 6.24.87$\pm$0.23 & 5.86$\pm$0.15\\
    %      \hline
    %      Humanoid & 1.03$\pm$0.15 & 4.16$\pm$ 0.39 & 6.29$\pm$0.64 & 6.02$\pm$0.48\\
    %      \hline
    %      Humanoid-Standup & 14.61$\pm$3.61 & 15.14$\pm$ 9.99 & 18.41$\pm$8.70 & 16.36$\pm$6.25\\
    %      \hline
    %      Walker & 2.93$\pm$0.52 & 2.66$\pm$0.77 & 6.24$\pm$0.33 & 5.15$\pm$0.33\\ [1ex] 
    %      \hline
    %     \end{tabular}
    %     }
    %     \caption{Performance of algorithms compared evaluated across 50 independent runs reported with $\pm 1 \ \mathsf{std\_dev}$}
    %     \label{table:results}
    % \end{table}
 
